Dark Matter, Millicharges, Axion and Scalar Particles, Gauge Bosons, and Other New Physics with LDMX

The proposed LDMX experiment would provide roughly a meter-long region of instrumented tracking and calorimetry that acts as a beam stop for multi-GeV electrons in which each electron is tagged and its evolution measured. This would offer an unprecedented opportunity to access both collider-invisible and ultra-short lifetime decays of new particles produced in electron (or muon)-nuclear fixed-target collisions. In this paper, we show that the missing momentum channel and displaced decay signals in such an experiment could provide world-leading sensitivity to sub-GeV dark matter, millicharged particles, and visibly or invisibly decaying axions, scalars, dark photons, and a range of other new physics scenarios.

==> authorabstract.tex <==
in% Philip

\author{Asher Berlin}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{Nikita Blinov}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{Gordan Krnjaic}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\author{Philip Schuster}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{Natalia Toro}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\begin{abstract}

The proposed LDMX experiment would provide roughly a meter-long region of instrumented tracking and calorimetry that acts as a beam stop for multi-GeV electrons in which each electron is tagged and its evolution measured. This would offer an unprecedented opportunity to access both collider-invisible and ultra-short lifetime decays of new particles produced in electron (or muon)-nuclear fixed-target collisions. In this paper, we show that the missing momentum channel and displaced decay signals in such an experiment could provide world-leading sensitivity to sub-GeV dark matter, millicharged particles, and visibly or invisibly decaying axions, scalars, dark photons, and a range of other new physics scenarios. 

\end{abstract}

